FreeToken: Efficient Edge-Native MoE Serving with Bandwidth-Adaptive Execution

Frontier open-weight models are increasingly available, but serving them still largely assumes datacenter infrastructure. We present FreeToken, an edge-native MoE serving system that treats a personal machine not as a small GPU, but as a unified, elastic inference platform. FreeToken co-designs the full serving stack, including model layout and loading, expert residency, CPU--GPU execution, agentic state reuse, and runtime memory management, around two realities of local AI: agent workloads continuously change their execution pattern, and edge hardware exposes heterogeneous resources whose balance differs from machine to machine. Rather than committing to a fixed offloading strategy, FreeToken continuously maps computation and model state onto the resources actually available. FreeToken supports more than 20 MoE models and real coding and tool-using agents across hardware ranging from an 8GB laptop GPU to a single workstation GPU. More importantly, it changes what these machines can practically serve, from a 35B model on a laptop to a 284B model on a gaming desktop and the 753B GLM-5.2 on a single workstation GPU. FreeToken turns open weights into deployable local software, making the machines users already own a practical platform for frontier-scale intelligence. We release the system at flashml.ai.

==> figure_texts/CachePolicy.tex <==
% Cache-policy comparison on identical routing traces; built at
% 0.85\textwidth. Placement in the paper TBD (5.2 locality or 5.4
% miss-policy ablation).
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/CachePolicy.pdf}
    \caption{Decode-time expert miss rate versus cache size under the
    three engines' placement policies, on identical routing traces.
    Lines are means over W1--W4, bands the min--max range.}
    \lblfig{cache-policy}
\end{figure}


==> figure_texts/CompileBenefits.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/CompileBenefits.pdf}
    \caption{Effectiveness of the \compileheuristic. \textbf{Left:} Compilation and configuration search time (log scale). The heuristic slashes tuning overhead by up to 175$\times$, entirely bypassing the severe compilation bottleneck of exhaustive auto-tuning. \textbf{Right:} Kernel iteration latency. The heuristic seamlessly matches the optimal performance found by exhaustive search across various shapes, ensuring near-zero runtime degradation.}
    \label{fig:compile_benefit}
\end{figure}

==> figure_texts/E2EBenchmark.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/E2EBenchmark.pdf}
    \caption{End-to-End Latency of \method compared to standard baselines. We group the evaluation into four representative regimes. The y-axis is presented in log scale to accommodate magnitude differences. Red \textbf{\texttimes} marks denote Out-Of-Memory failures (e.g., standard PyTorch fails to explicitly materialize the $N \times K$ distance matrix in Large $K$ workloads). \method delivers consistent and substantial speedups across diverse shapes and handles extreme limits gracefully.}
    \label{fig:e2e_benchmark}
\end{figure}

==> figure_texts/Exp2Prefill.tex <==
% Exp2 on its own row; built at 0.625\textwidth, included at
% 0.75\textwidth (1.2x: 7.5pt x tick labels print at 9pt).
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\textwidth]{figures/Exp2Prefill.pdf}
    \caption{Prefill TPS versus prompt length (RTX~5090, Qwen3.6-35B BF16)}
    \lblfig{exp2-prefill}
\end{figure}


==> figure_texts/KernelEfficiency.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/KernelEfficiency.pdf}
    \caption{Kernel-level latency breakdown. Latency comparison of our custom kernels versus standard implementations across diverse extreme workloads ($D=128$). \textbf{Left:} \FA completely removes HBM distance materialization, scaling up to a 21.2$\times$ speedup. \textbf{Right:} \SIU replaces per-token scatter atomic adds with sorted localized merges, eliminating atomic contention and achieving up to a 6.3$\times$ speedup.}
    \label{fig:kernel_speedup}
\end{figure}

==> figure_texts/PipelineAndAssign.tex <==
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{figures/PipelineAndAssign3.pdf} 
%     \caption{Illustration}
%     \label{fig:siu_mechanism}
% \end{figure*}

\begin{figure}[t]
    \centering
    % \includegraphics[width=0.8\textwidth]{figures/PipeAndAssign.pdf} 
    \includegraphics[width=0.8\textwidth]{figures/FlashAssignAndTime.pdf} 
    % \includegraphics[width=\textwidth]{figures/PipelineAndAssign3.pdf} 
    \caption{Overview of \method and Performance Breakdown.  
    (a) Inspired by IO-aware attention mechanisms, \FA streams data blocks from HBM to SRAM, fusing distance computation with an online argmin operator to completely bypass the materialization of the massive $N \times K$ distance matrix. 
    (b) Compared to standard \kmeans implementations, \method drastically compresses both the assignment IO bottleneck and the update synchronization bottleneck.}
    \label{fig:flash_kmeans_overview}
\end{figure}

==> figure_texts/SIUOverview.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/SIUOverview2.pdf} 
    \caption{Illustration of the centroid update stage and atomic contention. 
    \textbf{(a) Standard scatter-style update:} Tokens are directly scattered to their assigned centroids. The highly irregular mapping leads to severe write-side atomic contention when multiple threads update the same centroid simultaneously. 
    \textbf{(b) \Siu:} \method first sorts the tokens by their cluster IDs and constructs an inverse mapping. This transforms the unstructured scatter into regularized, segment-level localized reductions. 
    \textbf{(c) Execution timeline comparison:} The timeline reveals that the standard approach stalls frequently due to atomic lock contention on HBM, whereas \SIU issues contention-free memory writes, significantly hiding latency and accelerating the reduction phase.}
    \label{fig:siu_mechanism}
\end{figure*}

==> figure_texts/TierShowcase.tex <==
% Intro teaser: strongest servable model per hardware tier.
% Data: figures/src/data/tiershowcase.json (provenance inside).
\begin{figure}[t]
    \centering
    \includegraphics[width=0.72\textwidth]{figures/TierShowcase.pdf}
    \caption{On each consumer hardware tier, \FreeToken serves the
    strongest open-weight model that fits: Qwen3.6-35B (NVFP4) on an
    8\,GB laptop, DeepSeek-V4-Flash (284B, native MXFP4) on a
    32\,GB desktop, and GLM-5.2 (753B, NVFP4) on a single RTX PRO
    6000.  Bars give mean decode throughput on agentic workloads
    (coding agent on the first two tiers, math agent on the third);
    the dashed line marks the Codex median decode speed
    (33\,tok/s); \(\times\) marks engines that cannot serve the
    configuration.  \TODO{Cite the Codex median-speed source.}}
    \lblfig{tier-showcase}
\end{figure}


==> table_texts/Models.tex <==
\begin{table}[t]
    \centering
    \caption{Served models. Both checkpoints additionally store
    multi-token-prediction expert blocks (0.84B / 19B parameters)
    that never execute during serving and are excluded from the
    counts.}
    \lbltbl{models}
    \small
    \begin{tabular}{lcc}
        \toprule
        & Qwen3.6-35B-A3B & DeepSeek-V4-Flash \\
        \midrule
        Total / activated parameters & 35B / 3B & 284B / 13B \\
        Layers (all \MoE) & 40 & 43 \\
        Routed experts per layer & 256 & 256 \\
        Experts per token (top-\(k\) + shared) & 8 + 1 & 6 + 1 \\
        Expert weights & BF16 & MXFP4 \\
        Per-expert size & 6.3\,MB & 13.4\,MB \\
        Routed expert pool & 64.4\,GB & 147\,GB \\
        Attention / dense precision & BF16 & FP8 \\
        \bottomrule
    \end{tabular}
\end{table}


==> text/1_Introduction_v0.tex <==
\section{Introduction}
\lblsect{introduction}

\melissa{Agent is undoubtedly becoming the biggest workload for LLM \cite{70\% of anthropic revenue is from coding agent or something like that.}. While LLM now is very capable at a lot of tasks: delivering production code, pushing scientific frontier, x, such level of intelligence and capability is prohibitively expensive at scale for general public and only remains in enterprise and insitution. }




\TODO{P1--P5 below are a first prose draft for author/collaborator
iteration (per the 2026-07-18 meeting).  P6 remains an outline until
the evaluation and cost-analysis numbers exist.}

1. distinguish related work explicitly (emphasize our new techniques)
2. miss overhead is fundamental (fewer miss + faster transfer)
3. bullet points for top 3 techniques

The way people use language models is shifting from conversations to
agents: coding assistants that iterate against a repository for hours,
and tool-calling sessions that plan, execute, and retry autonomously.
Agents consume tokens in a way chat never did.  Anthropic reports an
average of \$150--250 per developer per month for its coding agent
across enterprise deployments, with heavy users exceeding \$1{,}000
monthly~\citep{claudecodecosts2026}, and independent accounts of
agent-heavy production workflows place the all-in figure several times
higher.  For individuals and small teams, continuous agentic use of
hosted frontier models is becoming prohibitively expensive.

Open-weight models look like the escape, but open weights are not open
access.  Serving a strong open model yourself calls for
enterprise-grade accelerators; renting it as tokens through hosted
APIs and gateways costs less than frontier subscriptions yet remains a
metered bill priced well above serving cost\TODO{one-clause margin
claim: verify the SemiAnalysis report before citing}---and either way,
private code and data still leave the machine.  The problem is not the
openness of the weights; it is affordable access to the intelligence
they contain.

What has quietly changed is how much of that intelligence now fits
locally servable sizes.  On the official benchmark suites, Qwen3.6-35B-A3B
---servable, as we show, from a laptop RTX 4060---outscores
MiniMax-M2.7, a 300B-class model; DeepSeek-V4-Flash, matched to
gaming-desktop GPUs from the RTX 3090 to the 5090, comes within one to
three points of GPT-5.2 on SWE-bench Verified and Pro---capability
that defined the closed-source frontier roughly half a year ago; and
GLM-5.2, an absolute-frontier open model, fits workstation cards of
the RTX Pro 6000 class.  \TODO{Verify the agent-arena rank of
DeepSeek-V4-Flash (author recalls first tier, $\approx$\#27).}  Each
of these models sits on the capability Pareto frontier of open
releases for its hardware tier.  The catch is that they are all \MoE
architectures: sparse activation puts their per-token computation
within a consumer \GPU's reach, but their expert pools exceed any
consumer \VRAM, and existing offloading engines leave them unusably
slow.  The capability exists; serving it does not.

\TODO{Teaser figure (Figure~1): capability-versus-time Pareto plot;
circle the three supported model/hardware tiers and annotate the
tokens/s \FreeToken achieves on each.  Needs strong visual impact.
Source data: arena/benchmark scores plus measured serving speeds.}

\FreeToken closes this gap by treating the central bottleneck---expert
weights that live in host memory rather than \VRAM---as a
bandwidth-allocation problem.  The complete expert pool resides in
\CPU memory and the \GPU caches complete experts; when routed experts
miss the cache, \FreeToken measures two properties of the deployed
machine, the effective expert-transfer bandwidth and the effective
host-side expert-processing bandwidth, and uses their balance to make
both decisions that miss service requires: whether to engage the \CPU
as a second execution path at all, and how many of the current misses
each path should receive (approximately \(q^\star\approx
m\,\BPcie/\BHost\) of \(m\) misses go to the transfer path).  When the
two bandwidths are close, every miss fills the cache; when host memory
outpaces the link, the \CPU absorbs the overflow using bandwidth the
saturated link cannot consume, while cache fills continue undisturbed.
Mode selection and workload division collapse into one measured
computation rather than two policies.

Turning this idea into a serving system imposes two further
requirements.  First, expert caching is inherently dynamic while fast
decode demands statically captured \CudaGraph execution, so \FreeToken
keeps all routing-dependent cache control on the \GPU, encodes dynamic
behavior as data inside a static graph, and captures the \CPU branch
itself through persistent workers and pinned buffers.  Second, edge
resources and workloads are not fixed: available \VRAM changes across
and within sessions, and agentic serving interleaves broad prefill
working sets with latency-critical decode over long multi-turn
sessions.  \FreeToken therefore manages expert memory as an elastic
resource---a runtime-resizable cache shared by prefill and decode, a
fast disk-to-host loading path, and a pure-\CPU boundary mode when
pinned memory is unavailable---inside a serving runtime with paged KV
management and prefix reuse, which multi-turn agentic sessions demand.

\TODO{P6 (outline; draft after results): scope sentence (``This report
describes the design, implementation, and evaluation of \FreeToken'');
four consumer GPUs, three FP4 models, agentic workloads, four
baselines; GLM-5.2 on RTX Pro 6000 as a separate demonstration, not a
full baseline matrix entry; direct capability contrast on the same
machine (what prior engines serve usably versus what \FreeToken
serves); cost analysis pricing a real coding-agent trace at API rates
for a capability-matched model versus \FreeToken on owned hardware,
reported as savings per month (no payback-period framing anywhere);
closing-line candidate: \FreeToken creates a new serving Pareto on
consumer hardware.}

